Competitive Online Optimization with Multiple Inventories: A Divide-and-Conquer Approach

We study a competitive online optimization problem with multiple inventories. In the problem, an online decision maker seeks to optimize the allocation of multiple capacity-limited inventories over a slotted horizon, while the allocation constraints and revenue function come online at each slot. The problem is challenging as we need to allocate limited inventories under adversarial revenue functions and allocation constraints, while our decisions are coupled among multiple inventories and different slots. We propose a divide-and-conquer approach that allows us to decompose the problem into several single inventory problems and solve it in a two-step manner with almost no optimality loss in terms of competitive ratio (CR). Our approach provides new angles, insights and results to the problem, which differs from the widely-adopted primal-and-dual framework. Specifically, when the gradients of the revenue functions are bounded in a positive range, we show that our approach can achieve a tight CR that is optimal when the number of inventories is small, which is better than all existing ones. For an arbitrary number of inventories, the CR we achieve is within an additive constant of one to a lower bound of the best possible CR among all online algorithms for the problem. We further characterize a general condition for generalizing our approach to different applications. For example, for a generalized one-way trading problem with price elasticity, where no previous results are available, our approach obtains an online algorithm that achieves the optimal CR up to a constant factor.

==> figs/related-tab.tex <==
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

 \begin{table}[htbp]
   \centering
   \caption{Comparison of our work and existing studies for online optimization under inventory constraints}
	\begin{tabular}{@{\extracolsep{4pt}}lccccc@{}}
	\hline
	\multicolumn{1}{c}{} & \multicolumn{3}{c}{Model} & \multicolumn{2}{c}{Results} \\ %\cline{2-4} \cline{5-6}
	 & Multi-entity & Concave-I & Concave-II & Optimal ($\theta=1)$ & Optimal ($\theta > 2^N)$  \\ \hline  %\bigstrut
	\cite{karp1990optimal,Devanur2013Randomized} & \cmark & \xmark & \xmark & \cmark & N/A \\
	\cite{lorenz2009optimal} & \xmark & \xmark & \xmark & \cmark & N/A \\
	\cite{aggarwal2011vertex,ma2020algorithms} & \cmark & \xmark & \xmark & \cmark & N/A \\
	\cite{KALYANASUNDARAM20003bmatching} & \cmark & \xmark & \xmark & \cmark & N/A \\ \hline
	\cite{el2001optimal} & \xmark & \xmark & \xmark & \cmark & \cmark \\
	\cite{Sun2020Competitive} & \cmark & \cmark & \xmark & \xmark & \xmark \\
	\cite{cr_pursuit2018} & \xmark & \xmark & \cmark & \cmark & \cmark \\
	Our work & \cmark & \cmark & \cmark & \cmark & \cmark \\ \hline
	\end{tabular}
  \label{tab:related}%
\end{table}%

%\begin{tabularx}{\linewidth}{clXXccXXXX}
%	\hline
%	 &  & \multicolumn{1}{l}{\cite{karp1990optimal,Devanur2013Randomized}} & \multicolumn{1}{l}{\cite{lorenz2009optimal}} & \cite{aggarwal2011vertex,ma2020algorithms} & \cite{KALYANASUNDARAM20003bmatching} & \cite{el2001optimal} & \cite{Sun2020Competitive} & \cite{cr_pursuit2018} & Our work \bigstrut \\ \hline
%	\multirow{3}{*}{Model} & Multi-entity & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark \\
%	 %& Continuous & \xmark & \xmark & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
%	 & Concave-I & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark \\
%	 & Concave-II & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark \\ \hline
%	\multirow{2}{*}{Results} & Optimal ($\theta=1)$ & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark \\  
%	 & Optimal ($\theta > 2^N)$ & N/A & N/A & N/A & N/A & \cmark & \xmark & \cmark & \cmark \\ \hline
%\end{tabularx}







%\newline
%\newline
%\begin{tabular}{|c|c|c|c|c|c|c|}
%	\hline
%		  & Entity & Profile & Work  & Tech. & Results & Opt. \bigstrut\\
%	\hline
%	\multirow{5}[4]{*}{Disc.} & \multirow{2}[2]{*}{Multiple} & \multirow{2}[2]{*}{Unweighted} & \cite{karp1990optimal},~\cite{Devanur2013Randomized} & P\&D  & $e/(e-1)$ & \multirow{6}[6]{*}{Tight} \bigstrut[t]\\
%		  &       &       & \cite{KALYANASUNDARAM20003bmatching} &       &  $1-(1-1/b)^b$ &  \bigstrut[b]\\
%	\cline{2-6}      & Single & Price Range & \cite{lorenz2009optimal} & RPP*  & charac. eqn. &  \bigstrut[t]\\
%		  & \multirow{2}[1]{*}{Multiple} & Singleton & \cite{aggarwal2011vertex} & P\&D  & $e/(e-1)$ &  \\
%		  &       & Price set & \cite{ma2020algorithms} &  P\&D & charac. eqn. &  \bigstrut[b]\\
%	\cline{1-6}\multirow{9}[12]{*}{Cont.} & Multiple & Unweighted & \cite{KALYANASUNDARAM20003bmatching} & Waterfilling & $e/(e-1)$ &  \bigstrut\\
%	\cline{2-7}      & \multirow{5}[6]{*}{Single} & linear & \cite{el2001optimal} & Threat-base & $\Omega(\ln\theta)$ & \multirow{3}[4]{*}{Tight} \bigstrut\\
%	\cline{3-6}      &       & \multirow{2}[2]{*}{Concave-I} & \cite{Sun2020Competitive} & P\&D  & \multirow{2}[2]{*}{$\ln\theta+1$} &  \bigstrut[t]\\
%	\cline{4-5}      &       &       & This work & CR-Pusuit &       &  \bigstrut[b]\\
%	\cline{3-7}      &       & \multirow{2}[2]{*}{Concave-II } & \cite{cr_pursuit2018} & CR-Pusuit & $\Omega(\ln\theta)$ & Order \bigstrut[t]\\
%	\cline{4-7}
%		  &       &       & \cite{Sun2020Competitive} & P\&D  &  $\ln\theta+\Omega(1)$& Near \bigstrut[b]\\
%	\cline{2-7}      & \multirow{3}[4]{*}{Multiple} & Concave -I & \cite{Sun2020Competitive} & P\&D  & $<\ln\theta+2$ & Near \bigstrut\\
%	\cline{3-7}      &       & Concave-I & \multirow{2}[2]{*}{This work} & Divede- & $<\ln\theta+2$ & Near \bigstrut[t]\\
%	  \cline{6-7}    &       & Concave-II  &       & and-conquer & $\Omega(\ln\theta)$ & Order \bigstrut[b]\\
%	\hline
%\end{tabular}


==> figs/result-sum.tex <==

\begin{table}[htbp]
	\centering
	\begin{tabular}{lll}
		\hline
		 & Single-entity & Multiple-entity \bigstrut \\ \hline
		Concave-I & $\ln \theta + 1^\star$ & $<\ln \theta + 2^{\#}$ \bigstrut \\
		Concave-II &  $\ln \theta + 1^\star$ & $\Omega (\ln \theta)$ \bigstrut\\ \hline  
	\end{tabular}	
	\\\footnotesize{$^\star$: CR is optimal. \quad
		$^\#$: CR is optimal when $\theta=1$ or $\theta > 2^{N-1}$. 
	}
	\caption{Results summary of our method}
\end{table}
